Learning Optical Flow for Fast MRI Reconstruction

Reconstructing high-quality magnetic resonance images (MRI) from undersampled raw data is of great interest from both technical and clinical point of views. To this date, however, it is still a mathematically and computationally challenging problem due to its severe ill-posedness, resulting from the highly undersampled data leading to significantly missing information. Whilst a number of techniques have been presented to improve image reconstruction, they only account for spatio-temporal regularisation, which shows its limitations in several relevant scenarios including dynamic data. In this work, we propose a new mathematical model for the reconstruction of high-quality medical MRI from few measurements. Our proposed approach combines - \textit{in a multi-task and hybrid model} - the traditional compressed sensing formulation for the reconstruction of dynamic MRI with motion compensation by learning an optical flow approximation. More precisely, we propose to encode the dynamics in the form of an optical flow model that is sparsely represented over a learned dictionary. This has the advantage that ground truth data is not required in the training of the optical flow term. Furthermore, we present an efficient optimisation scheme to tackle the non-convex problem based on an alternating splitting method. We demonstrate the potentials of our approach through an extensive set of numerical results using different datasets and acceleration factors. Our combined approach reaches and outperforms several state of the art techniques. Finally, we show the ability of our technique to transfer phantom based knowledge to real datasets.

==> img/results/cine/cine_figure.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% File to produce the figure with the results of the CINE Dataset
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
%           | Fully Sampled | 4x | 6x | 8x | 
% IFT       |
% CS        |
% CS+TVL1   |
% MC+JPDAL  |
% DLMC+R    |
%% 

% \begin{figure}[!h]
%     \centering
%     %% Inverse Fourier transformed
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/references/cine_r_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/results/cine/zf/cine_zf_4_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/results/cine/zf/cine_zf_6_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/results/cine/zf/cine_zf_8_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \\ %%% Pure Compressed Sensing 
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/references/cine_r_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/results/cine/cs/cine_cs_4_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/results/cine/cs/cine_cs_6_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/results/cine/cs/cine_cs_8_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%      \\ %%% Compressed Sensing + TVL1 
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/references/cine_r_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/results/cine/cstvl1/cine_cstvl1_4_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/results/cine/cstvl1/cine_cstvl1_6_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/results/cine/cstvl1/cine_cstvl1_8_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \\ %%% CS + JPDAL
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/references/cine_r_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/results/cine/mcjpdal/cine_mcjpdal_4_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/results/cine/mcjpdal/cine_mcjpdal_6_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/results/cine/mcjpdal/cine_mcjpdal_8_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \\ %%% DLMC + R
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/references/cine_r_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/results/cine/dlmcr/cine_dlmcr_4_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/results/cine/dlmcr/cine_dlmcr_6_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/results/cine/dlmcr/cine_dlmcr_8_frame_1.jpg}
%         % \caption{CINE}
%         % \label{sub-fig:cine_reference}
%     \end{subfigure}
%     \caption{The first row is the reference first frame for the four datasets, the rows 2-3-4 correspond to the same frame degraded with masks}
%     \label{fig:cine_results}
% \end{figure}

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=\textwidth]{    \includegraphics[width=\textwidth]{}

% }
% \end{figure}

==> img/results/undersampled_fig.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% File to produce the figure with the different datasets
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}
%      \centering
%      %%% REFERENCES
%      \begin{subfigure}[b]{0.2\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{img/references/cine_r_frame_1.jpg}
%          \caption{CINE}
%          \label{sub-fig:cine_reference}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.2\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{img/references/eth_r_frame_1.jpg}
%          \caption{ETH}
%          \label{sub-fig:eth_reference}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.2\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{img/references/phantom_bh_r_frame_1.jpg}
%          \caption{PHANTOM Breath Holding}
%          \label{sub-fig:phantom_bh_reference}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.2\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{img/references/phantom_fb_r_frame_1.jpg}
%          \caption{PHANTOM Free Holding}
%          \label{sub-fig:phantom_fb_reference}
%      \end{subfigure}     
%      \\ %%% UNDERSAMPLED 4
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/undersampled/acc_4/cine_zf_4_frame_1.jpg}
%         \caption{CINE}
%         \label{sub-fig:cine_acc_4}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/undersampled/acc_4/eth_zf_4_frame_1.jpg}
%         \caption{ETH}
%         \label{sub-fig:eth_acc_4}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/undersampled/acc_4/phantom_bh_zf_4_frame_1.jpg}
%         \caption{PHANTOM Breath Holding}
%         \label{sub-fig:phantom_bh_acc_4}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/undersampled/acc_4/phantom_fb_zf_4_frame_1.jpg}
%         \caption{PHANTOM Free Holding}
%         \label{sub-fig:phantom_fb_acc_4}
%      \end{subfigure}     
%      \\ %%% UNDERSAMPLED 6
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/undersampled/acc_6/cine_zf_6_frame_1.jpg}
%         \caption{CINE}
%         \label{sub-fig:cine_acc_6}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/undersampled/acc_6/eth_zf_6_frame_1.jpg}
%         \caption{ETH}
%         \label{sub-fig:eth_acc_6}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/undersampled/acc_6/phantom_bh_zf_6_frame_1.jpg}
%         \caption{PHANTOM Breath Holding}
%         \label{sub-fig:phantom_bh_acc_6}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/undersampled/acc_6/phantom_fb_zf_6_frame_1.jpg}
%         \caption{PHANTOM Free Holding}
%         \label{sub-fig:phantom_fb_acc_6}
%      \end{subfigure}        
%      \\ %%% UNDERSAMPLED 8
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/undersampled/acc_8/cine_zf_8_frame_1.jpg}
%         \caption{CINE}
%         \label{sub-fig:cine_acc_8}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/undersampled/acc_8/eth_zf_8_frame_1.jpg}
%         \caption{ETH}
%         \label{sub-fig:eth_acc_8}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/undersampled/acc_8/phantom_bh_zf_8_frame_1.jpg}
%         \caption{PHANTOM Breath Holding}
%         \label{sub-fig:phantom_bh_acc_8}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/undersampled/acc_8/phantom_fb_zf_8_frame_1.jpg}
%         \caption{PHANTOM Free Holding}
%         \label{sub-fig:phantom_fb_acc_8}
%      \end{subfigure}        
%     \caption{The first row is the reference first frame for the four datasets, the rows 2-3-4 correspond to the same frame degraded with masks: 25\%, 16\% and 12.5\%}
%     \label{fig:datasets_reference}
% \end{figure}


%%% From the results in github I propose the following figures: 

%%Unfinished fig. doing the diff maps
%\begin{figure*}[t!]
%\centering
%\includegraphics[width=1\textwidth]{img/Figs.Out/comparisonA.pdf}
%\caption{}
%\label{fig::CSvsCSPlusM}
%\end{figure*}
%it is missing the maps


==> sections/1_related_works.tex <==
%\textcolor{red}{[Noemie] Related Work:  please let me know if you don't like the flow or this section doesn't match what you had in mind} \textcolor{blue}{Can we separate the long paragraphs in more short ones? We need to reduce and spend time in related work from optical flow (particular in recognised the learning optical flow). We can remove for instance paragraph 1 as the idea is in the introduction and reduce the following ones. }
%\textcolor{red}{I see that the flow and the ideas of the introduction and the related work section are very similar. I think it would be a good idea to merge both sections into a bigger introduction. It is also very common to have only the introduction section in SIAM papers and not related works. Tell me what you think. Thanks :)}\\
In this section, we review the literature in turn related three key parts of our technique: i) Fast MRI reconstruction, ii) Learning Optical Flow and iii) Joint Models. 

\medskip
\textit{Fast MRI reconstruction.} The problem of reconstructing high quality images, from dynamic Magnetic Resonance (MR) measurements, whilst reducing the inherent involuntary motion during the acquisition is a central topic in the community. Although it has been widely explored, it is still considered an open problem. This central topic in MRI comes as a consequence of the long acquisition time, which makes the image formation highly sensitive to motion leading to image degradation and compromising the expert interpretation \cite{sachs1995diminishing,Zaitsev::2015}. 
%One has to distinguish between intra-frame motion happening during individual MR experiments and inter-frame motion occurring between individual MR experiments. In this work, we focus on inter-frame motion only. In this section, we review the existing techniques of dynamic MRI sequences without providing an exhaustive survey which goes beyond the scope of this paper.

There are several attempts in the body of literature, to improve the reconstruction under inherent motion. A set of solutions to reduce motion artefacts include breath-holding techniques \cite{plathow2006assessment,Zaitsev::2015,gdaniec2014robust} and gating strategies \cite{Setser2000,Plein2001,Kaji2001,GEORGE2006924,JIANG2006141,Zaitsev::2015}.
The former rely on the  patients' ability to hold their breath. However, the time needed to form an image is much longer than the average time a human being is capable of holding its breath%of the human breath-holding
~\cite{plathow2006assessment}. The latter aim at tracking either the breathing or the cardiac cycles. However, the co-registration of these signals to the image ones is still challenging ~\cite{HOISAK2006339,Zaitsev::2015} and these techniques are effective only for perpetual motions disregarding any other involuntary motion or arrhythmia \cite{Zaitsev::2015} and thus are only partially accurate.

%Classical ways to reduce motion artefacts include breath-holding techniques \cite{plathow2006assessment,zaitsev2015motion,gdaniec2014robust} and gating strategies \cite{Setser2000,Plein2001,Kaji2001,GEORGE2006924,JIANG2006141,zaitsev2015motion}.
%The former depend on the patients' ability to hold their breath for as much time as possible and therefore are limited \cite{plathow2006assessment}. Residual physiological motion are likely to happen before dynamic scan is complete. Successive breath holds can also be done but the variability between breath holds is still responsible for residual artefacts and this technique requires longer time for the full scan to be done. 
%The latter aim at tracking either the breathing or the cardiac cycles and grouping the measurements according to the cycle phase during which they are taken via external sensors. However, the co-registration of these signals to the image ones is still challenging \cite{HOISAK2006339,zaitsev2015motion} and these techniques are effective only for perpetual motions disregarding any other involuntary motion or arrhythmia \cite{zaitsev2015motion} and thus are only partially accurate.

The idea of accelerating the MRI acquisition by using under-sampling strategies is an alternative to the aforementioned techniques. This option has %been focus of
gained great interest particularly because of the advent of Compressed Sensing (CS) in MRI~\cite{lustig2007}. CS relies on the property of MR images to be sparse in a transformed domain. Examples are  \cite{LustigktSPARSE::2006,Otazo::2010,LustigSPIRiT::2010,lingala::2013,Liang::2007,gamper2008compressed,jung2009k,Lingala::2011}, in which authors applied several known or learned transformations alone or in combination with parallel imaging. Another set of works has been devoted to extend the idea of CS, and is based on low-rank matrix completion by taking advantage of the highly redundant information present in dynamic MRI sequences. For example, the work of Liang~\cite{Liang::2007}, in which a singular value decomposition (SVD) is used to compute the temporal basis functions, has paved the way to techniques relying on Principal Component Analysis (PCA) to reconstruct from under-sampled measurements \cite{Pedersen::2009,Feng::2013,Velikina::2015,arif2019accelerated}. Other works have proposed to incorporate local low rank constraints in small regions to reduce the computational load \cite{Trzasko::2011,Zhang::2015,Miao::2016}. However they come at the expense of block artefacts \cite{Saucedo::2017}.

%As an alternative to these techniques, the idea of accelerating the MRI acquisition by using under-sampling strategies while keeping a high quality image reconstruction has gained a lot of interest. Especially, the potentials and benefits of Compressed Sensing to reconstruct dynamic MR sequences from under-sampled measurements has been demonstrated in many works since the seminal paper by Lustig \cite{lustig2007}. It relies on the property of MR images to be sparse in a transformed domain. Many transformations have been applied in \cite{LustigktSPARSE::2006,Otazo::2010,LustigSPIRiT::2010,lingala::2013,Liang::2007,gamper2008compressed,jung2009k,Lingala::2011} alone or in combination with parallel imaging and with known transformations or unknown ones that are simultaneously estimated.
%Another line of search in this area extending the previous ideas is based on low-rank matrix completion by taking advantage of the highly redundant information present in dynamic MRI sequences. A new way to reconstruct dynamic MR sequences from under-sampled measurements was proposed by Liang in \cite{Liang::2007} in which a singular value decomposition (SVD) is used to compute the temporal basis functions. This work has paved the way to techniques relying on Principal Component Analysis (PCA) to reconstruct from under-sampled measurements \cite{Pedersen::2009,Feng::2013,Velikina::2015}; and to the work of Asif et al. \cite{arif2019accelerated} introducing a reconstruction framework that simultaneously learns the temporal basis functions and the spatial weights of the kernel-induced feature space via a kernel-based low rank constraint to efficiently use the nonlinear correlation in the dynamic sequence. These techniques apply global low rank constraints but other works have proposed to incorporate local low rank constraints exploiting the spatiotemporal correlation in small regions to reduce the computational load \cite{Trzasko::2011,Zhang::2015,Miao::2016}. However they come at the expense of block artefacts \cite{Saucedo::2017}.

A body of researches has proposed to combine sparse and low-rank constraints e.g.~\cite{Lingala::2011,Majumdar::2012,Zhao::2012}. Another approach consists in decomposing the reconstruction into a sparse component and a low rank one known as both Robust Principal Component Analysis (RPCA) \cite{Candes::2011} and L+S decomposition \cite{Gao::2012,Tremoulheac::2014,Otazo::2013,Otazo::2015}. Even though the efficiency of these techniques has been proved in the context of dynamic MRI reconstruction, the incoherence required for the L+S decomposition is not always fulfilled. The success of these models is promising but there is still room for improvement as they do not take into account the explicit motion exhibited during the dynamic acquisition. Thus reconstruction techniques also considering this motion have emerged to improve the quality of the reconstructed sequence in a dynamic setting. 
%Before introducing motion estimation into the reconstruction process, one needs to answer the fundamental question of \textit{how to appraise the inter-frame motion?} There are mainly two strategies based either on registration \cite{sotiras2013} or on optical flow \cite{fortun2015}. In this work, we focus on the latter and therefore review some of the previous works dedicated to solving the optical flow problem. Assuming brightness constancy, it consists in estimating the velocities of movement of brightness patterns in an image. Relying on this assumption only, the optical flow is a very ill-posed problem due to the aperture problem. The seminal paper by Horn and Shunck \cite{horn1981} introduced a variational formulation of the problem comprising an $L^2$ fidelity term coming from the linearised brightness constancy assumption and an $L^2$ regularity term on the flow fields to ensure smoothness and make the problem well-posed. Since then, there has been a large body of works trying to improve the quality and the accuracy of the obtained flows in a variational setting \cite{fortun2015}. They especially include the work of Perez et al. \cite{perez2013} known as the $TV-L^1$ model in which the $L^2$ norms are replaced by $L^1$ ones to allow discontinuities of the flow fields at object boundaries, and nonlocal variants \cite{sun2010secrets,dong2014}. 


\textit{Motion Estimation.} There are two popular strategies for motion estimation based either on registration \cite{sotiras2013} or optical flow \cite{fortun2015}. In this work, we focus on the latter. Optical flow relies on the  brightness constancy assumption, and consists in estimating the velocities of movement of brightness patterns in an image. Optical flow is a very ill-posed problem due to the aperture problem. %First solutions to this problem were casted the OF as a variational approach, starting with the seminal work of that  Shunck \cite{horn1981}. 
First, variational approaches were introduced to solve the OF problem, starting with the seminal work of Horn and Schunck \cite{horn1981}.
In that work, authors introduced an $L^2$ fidelity term coming from the linearised brightness constancy assumption and an $L^2$ regularity term on the flow fields to ensure smoothness and make the problem well-posed. Since then, there has been a large body of works trying to improve the quality and the accuracy of the obtained flows in a variational setting \cite{fortun2015,perez2013}.
\textcolor{red}{to add a bunch of approaches for OF. Are you sure, I put a review to avoid citing too many papers....}

More recently, several authors have explored the optical flow problem using tools drawn from machine learning. Astonishing results have been reported using deep learning either for normal scene conditions e.g.\cite{sun2018pwc,dosovitskiy2015flownet,ilg2017flownet} or extreme scenarios e.g.\cite{li2019rainflow}. We remark that our purpose in this work is different from those works. Whilst they aim to improve the optical flow estimation itself, \textit{our goal is instead to use OF as proxy to improve the MRI reconstruction.} In particular, we are interested in learning the optical flow using sparse coding. Our motivation to follow this philosophy, is given by the promising results reported in image restoration e.g~\cite{elad2006image,mairal2009non}. The central idea of sparse coding is to find a dictionary such that each measurement can be well-approximated by a sparse linear combination of atoms (i.e. elements of a dictionary).

There have been several attempts to learn a sparse optical flow. The works of that~\cite{timofte2015sparse,shen2010sparsity}  used known basis functions whilst authors in~\cite{jia2011} learned an overcomplete dictionary coming either from ground truth set or from classic variational estimation \cite{gibson2016sparsity,wulff2015efficient}. The major drawback of these techniques is the lack of convergence guarantee but this has been overcome by the work of Bao~\cite{bao2015dictionary}. In that work, authors introduced a globally convergent algorithm to solve generic dictionary learning and sparse coding problems. Whilst sparse coding has been widely explored for natural images, sparse optical flow models have yet to be tackled in the medical domain and only few works have been reported e.g.~\cite{ouzir2018robust}. 


\textit{Joint Models.} We remark that our ultimate goal is to improve the image reconstruction for dynamic MRI sequences. To this purpose, we include motion estimation as proxy for improving MRI reconstruction. Following this perspective, different works have been reported using so-called joint models, in which  the main idea is to intertwine several related tasks into a single unified functional. The potential in terms of image quality improvement whilst reducing error propagation has been shown in~\cite{aviles2018, liu2019rethinking,caruana1997multitask,Zhao::2019}.
There are several works that follow this idea either for reconstructing a single image e.g.\cite{odille2008generalized,Corona::2019,weller2019motion,Prieto::2007,haskell2018targeted} or a full image sequence e.g.~\cite{Bilen::2011,Usman::2013,bustin2016motion,Odille::2010}.
\textcolor{red}{check references}

%In the body of literature has been reported other works that rely on prior and external knowledge to generate motion models from sensors, navigators, etc. \cite{Odille::2016} or driven by previously computed eigenmodes of cardiac and respiratory motions \cite{Odille::2010}.

Authors of that \cite{Lingala::2015} proposed the self-contained Deformation Corrected-Compressed Sensing (DC-CS) model relying on CS principles along with a Demons algorithm to estimate the motion. More recently, Zhang et al. in~\cite{Zhang::2018} extended this model to the concept of Blind Compressed Sensing, in which the transformation leading to sparsity is also estimated. In particular, our proposed approach follows the same perspective as the works of \cite{aviles2018,Zhao::2019,burger2018}, in which CS and OF principles are combined. We emphasise that the main difference stands in the optical flow formulation. That is- we propose a new optimisation model, in which the flow estimation is encoded in a sparse representation over a learnt dictionary.  \textcolor{blue}{*to add minor comment  ** we can also reduce Fast  MRI  reconstruction part from the related work}


%In \cite{Zhao::2019}, the authors introduce a joint CS reconstruction and affine optical flow model in which the weighted optical flow task is simplified by considering only affine displacement fields. Whilst \cite{burger2018} provides an extensive theoretical analysis of a joint CS reconstruction and full optical flow model without MR applications, our work introduces a new formulation of the model in which the displacement fields are learnt from a dictionary with sparse coding and focuses on dynamic MRI applications. 




%With the expansion of sparse coding showing great potentials in many computer vision applications, many works were devoted to the application of this technique to the optical flow problem first using known basis functions \cite{timofte2015sparse,shen2010sparsity} and then learned ones from an overcomplete dictionary coming either from groundtruth \cite{jia2011} or from classic variational estimation \cite{gibson2016sparsity,wulff2015efficient}. Surprisingly, the latter have shown better results than the original model used to learn the dictionary. The major drawback of these techniques is the lack of convergence guarantee but this has been overcome by the work of Bao et al. \cite{bao2015dictionary} in which they introduce a globally convergent algorithm to solve generic dictionary learning and sparse coding problems. More recently, deep learning based approaches have thrived and been successfully applied to the optical flow problem in normal conditions \cite{sun2018pwc,dosovitskiy2015flownet,ilg2017flownet} or in extreme conditions like heavy rain \cite{li2019rainflow,}. We can now integrate this motion estimation in the MRI reconstruction model to improve the final image quality.\\
%Different strategies have been explored in this regard including \cite{odille2008generalized,Corona::2019,weller2019motion,Prieto::2007,haskell2018targeted} in which the final goal is to reconstruct a single image. But in this work, we aim at reconstructing the whole sequence. With this in mind, a natural way to incorporate the motion information in the reconstruction framework is by a sequential scheme in which a classical reconstruction is performed followed by a motion estimation step including rigid, affine and deformable registration techniques and finally the images are refined by a motion-corrected reconstruction as in \cite{Bilen::2011,Usman::2013,bustin2016motion,odille2010model}. 

%% NOTE to discuss :: 
%Another lead consists in deriving an iterative scheme solving two coupled inverse problems but not coming from the same original optimisation problem with one dedicated to the estimation of the motion and the other devoted to the motion-informed reconstruction of the MR sequence \cite{royuela2016nonrigid,Royuela::2017,filipovic2011motion,Asif::2013,Rank::2017}. 


%Finally, as sharing representation between tasks in a unified and joint optimisation problem has shown great potential to improve the quality of the results and to reduce error propagation \cite{aviles2018, liu2019rethinking,caruana1997multitask,Zhao::2019,liu2019rethinking}, scientists have introduced joint models to simultaneously reconstruct the whole dynamic MRI sequence and estimate the inter-frame motion. 
%Some of them rely on prior and external knowledge to generate motion models from sensors, navigators, etc. \cite{Odille::2016} or driven by previously computed eigenmodes of cardiac and respiratory motions \cite{Odille::2010}. Authors of that \cite{Lingala::2015} proposed the self-contained Deformation Corrected-Compressed Sensing (DC-CS) model relying on CS principles along with a Demons algorithm to estimate the motion. Most recently, Zhang et al. extended this model to the concepts of Blind Compressed Sensing \cite{Zhang::2018} in which the transformation leading to sparsity is also estimated. Finally, our model follows the philosophy of that \cite{Zhao::2019} and \cite{burger2018} combining CS and Optical Flow (OF) principles. We emphasise that the main difference stands in the optical flow formulation. In \cite{Zhao::2019}, the authors introduce a joint CS reconstruction and affine optical flow model in which the weighted optical flow task is simplified by considering only affine displacement fields. Whilst \cite{burger2018} provides an extensive theoretical analysis of a joint CS reconstruction and full optical flow model without MR applications, our work introduces a new formulation of the model in which the displacement fields are learnt from a dictionary with sparse coding and focuses on dynamic MRI applications. 
